Additive Control Variates Dominate Self-Normalisation in Off-Policy Evaluation

Off-policy evaluation (OPE) is essential for assessing ranking and recommendation systems without costly online interventions. Self-Normalised Inverse Propensity Scoring (SNIPS) is a standard tool for variance reduction in OPE, leveraging a multiplicative control variate. Recent advances in off-policy learning suggest that additive control variates (baseline corrections) may offer superior performance, yet theoretical guarantees for evaluation are lacking. This paper provides a definitive answer: we prove that $\beta^\star$-IPS, an estimator with an optimal additive baseline, asymptotically dominates SNIPS in Mean Squared Error. By analytically decomposing the variance gap, we show that SNIPS is asymptotically equivalent to using a specific -- but generally sub-optimal -- additive baseline. Our results theoretically justify shifting from self-normalisation to optimal baseline corrections for both ranking and recommendation.

==> appx_old.tex <==
\section{Introduction \& Motivation}

Self-normalised importance sampling~\cite[\S 9]{Owen2013} is great: SNIPS.
Importance sampling with baseline corrections~\cite{Gupta2024} is also great: $\beta$-IPS.

In off-policy learning scenarios, there is an equivalence between optimising for SNIPS and $\beta$-IPS: it boils down to the choice of $\beta$ (cfr. BanditNet~\cite{Joachims2018}).
Granted, it is unclear what exact value of $\beta$ gives us an estimator with an equivalent maximum to SNIPS, but because \citet{Gupta2024} derive the optimal (variance-minimising) values of $\beta$, we know that it could never be better than using $\beta^{\star}$.

That leaves off-policy evaluation, and the question whether SNIPS (with its multiplicative control variate and asymptotic unbiasedness) is equivalent to an instantiation of $\beta$-IPS (with its additive control variate and finite-sample unbiasedness).
If we can show that this is indeed the case, we can essentially disregard SNIPS as an evaluation method, as $\beta$-IPS has both improved bias and improved variance.
\textcolor{Green}{BL: This could use some clarification. The $\beta^\star$ baseline correction given by $\beta$-IPS has the minimal variance of all baseline corrections. So if we can show that SNIPS is equivalent to \emph{some} baseline correction, then we know that it yields only at best the same variance as $\beta$-IPS. Right? Is that it?}
\textcolor{Maroon}{OJ: Yep! }

There are two arguments to be made here, which we lay out mathematically.
We start with the one that is conceptually simpler, because we can refer to existing results; and then proceed with the more general case.

\subsection{Pairwise Comparisons}
We want to assess differences in average obtained reward for two competing policies: $\pi$ and $\pi^{\prime}$.
Our estimand is:
\begin{equation}
    V_{\Delta}(\pi,\pi^{\prime}) = \mathbb{E}_{a \sim \pi}[R] - \mathbb{E}_{a \sim \pi^\prime}[R].
\end{equation}
In the absence of A/B-test data but with data collected under some stochastic logging policy $\pi_0$, the two terms on the right-hand side of this equation are typically estimated with off-policy estimators~\cite{Jeunen2024_DeltaOPE}---for example, SNIPS~\cite{Swaminathan2015}.
For completeness, this gives:
\begin{equation}\label{eq:delta_snips}
   V_{\Delta{\rm -SNIPS}}(\pi,\pi^{\prime}) = \underbrace{\frac{\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi(a|x)}{\pi_0(a|x)}R\right]}{\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi(a|x)}{\pi_0(a|x)}\right]}}_{V(\pi)} - \underbrace{\frac{\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi^{\prime}(a|x)}{\pi_0(a|x)}R\right]}{\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi^{\prime}(a|x)}{\pi_0(a|x)}\right]}}_{V(\pi^{\prime})}.
\end{equation}

To assess which policy yields the highest expected reward, a statistical test is then carried out on an empirical estimate, in an attempt to reject the no-effect null hypothesis $V_{\Delta{\rm -SNIPS}}(\pi,\pi^{\prime})=0$.

This procedure is the offline evaluation equivalent to common online evaluation practices, i.e. A/B-testing~\cite{kohavi2020trustworthy}.
Several parallels can be drawn between these two paradigms. 
Regression adjustments~\cite{Freedman2008}, where some learned model of expected reward is used as an additive control variate to reduce the variance in observed rewards, appears both in A/B-testing~\cite{Deng2013,Poyarkov2016} as well as in off-policy estimation, referred to as ``doubly robust'' methods~\cite{Dudik2014}.
To deal with ratio metrics, where the estimand is not expressed a single expectation over randomisation units (e.g. click-through-rate), the delta method is used to approximate variance~\cite[\S 11]{Lehmann2005}---which directly carries over to SNIPS~\cite{Swaminathan2015}.
Specialised methods that combine ratio estimates with regression adjustments have been proposed too, for A/B-testing~\cite{Budylin2018, Baweja2024} as well as off-policy evaluation~\cite{Thomas2016,Kallus2019}.

Of particular interest is the work of \citet{Budylin2018}, showing that all ratio metrics can be transformed into linearised versions of the form ``${\rm numerator} - \alpha \cdot  {\rm denominator}$''.
Furthermore, these linearised versions come with strong theoretical guarantees on both
\begin{enumerate*}[label=(\roman*)]
    \item \emph{directionality}, and 
    \item \emph{sensitivity} of the metric.
\end{enumerate*}

Their argument translates directly to Eq.~\ref{eq:delta_snips}.
Hence: we can obtain a linearised version of the SNIPS estimator that is guaranteed to retain its directionality as well as its sensitivity \emph{in pairwise comparisons}.
A linearised version of SNIPS would become:
\begin{align}
    V_{\rm L-SNIPS}(\pi) &=\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi(a|x)}{\pi_0(a|x)}R\right] -\alpha \mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi(a|x)}{\pi_0(a|x)}\right] \nonumber \\
    &=\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi(a|x)}{\pi_0(a|x)}R\right] -\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi(a|x)}{\pi_0(a|x)}\alpha \right] \nonumber \\
    &=\mathop{\mathbb{E}}\limits_{a \sim \pi_0}\left[\frac{\pi(a|x)}{\pi_0(a|x)}(R-\alpha)\right].
\end{align}
\textcolor{Blue}{SG: **Very first thought, will read more in detail in the next few days for more detailed comments** 1) Do the guarantees on directionality and sensitivity hold for a particular value of $\alpha$? \textcolor{Maroon}{[OJ: yes, directionality holds for a range and the sensitivity result is proven for $\alpha=\hat V_{\rm SNIPS}(\pi)$. This is interesting, I seem to remember from our RecSys '24 draft and musings that we found something like this: SNIPS is equivalent to beta-SNIPS when beta is equal to the SNIPS estimator itself.]} Are $\alpha$ and $\beta$ related in any way? Is the relation interesting/useful? \textcolor{Maroon}{[Unsure, really.]} 2) The linearised version of SNIPS is equivalent in the sense of directionality and sensitivity, which is useful for off-policy paired comparison, as you said before this section? How about it's unbiasedness? \textcolor{Maroon}{[Should be unbiased, as it boils down to \cite[Eqs. 16--17]{Jeunen2024_DeltaOPE}]} Or equivalence in terms of absolute values? I see that you show equivalence in terms of Taylor-series expansion later. I'll read more in detail later. 3) Adding an $\alpha$ in eq. 3 will lead to an **unbiased linearized SNIPS** estimator (unless it changes the directionality guarantees?). }
Here, $\alpha$ works as a baseline correction, implying an equivalence between $V_{\rm L-SNIPS}$ and $V_{\beta{\rm -IPS}}$~\cite{Gupta2024}.
The results from \citet{Budylin2018} only relate to pairwise comparisons, hence providing guarantees on preserved directionality and significance between $V_{\Delta{\rm L-SNIPS}}$ and $V_{\Delta\beta{\rm -IPS}}$~\cite[Eq.~16]{Jeunen2024_DeltaOPE}.
By transitivity, we have an equivalence between $V_{\Delta{\rm-SNIPS}}$ and $V_{\Delta\beta{\rm -IPS}}$.
As \citet{Jeunen2024_DeltaOPE} characterise the optimal variance-minimising value of $\beta$, this implies that $V_{\Delta\beta{\rm -IPS}}$ will always offer either an improvement over $V_{\Delta{\rm-SNIPS}}$ or an equivalence, when the linearisation hyperparameter $\alpha$ coincides with the optimal $\beta$ that is computed via closed-form expression.

This is a strong and important result that applies to pairwise comparisons between policies.
In what follows, we additionally argue a more fundamental result, proving an equivalence between the stand-alone estimators.

\textcolor{Maroon}{\it
I suppose if I dig into the math from \citet{Budylin2018}, their sensitivity result must also hold for the standalone estimates for the policies $\pi, \pi^\prime$ and not only the treatment effect? I suppose to enunciate that clearly, I need to actually understand all of it, and it's a pretty dense paper and proof.
}


\subsection{Standalone Estimators}
An empirical SNIPS estimate on logged data $\mathcal{D}$ is given by the ratio:
\begin{equation}
    \hat{V}_{\rm SNIPS}(\pi) = \frac{\sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a|x)}{\pi_0(a|x)}r}{\sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a|x)}{\pi_0(a|x)}} = \frac{\sum_{(x,a,r) \in \mathcal{D}} y}{\sum_{(x,a,r)\in\mathcal{D}}w}= \frac{\bar{Y}}{\bar{W}}.
\end{equation}
For mathematical notational convenience, we define $w\equiv \frac{\pi(a|x)}{\pi_0(a|x)}$ and $y\equiv wr$.
It is common to simplify this ratio through a first-order Taylor expansion, usually to obtain a variance estimate (i.e. the delta method).
\textcolor{Green}{BL: Don't you need the expected value of SNIPS on the lefthand side? Otherwise, these expectations on the right are empirical, no? And in that case, the average of $w$ is not 1.}
This results in:
\begin{align}
\hat{V}_{\rm SNIPS} &\approx \frac{\mathbb{E}[y]}{\mathbb{E}[w]} + \frac{1}{\mathbb{E}[w]}(\bar{Y} - \mathbb{E}[y]) - \frac{\mathbb{E}[y]}{(\mathbb{E}[w])^2}(\bar{W} - \mathbb{E}[w]) \nonumber \\
&\approx \mathbb{E}[y] + (\bar{Y} - \mathbb{E}[y]) - \mathbb{E}[y](\bar{W} - 1)\nonumber\\
&= \bar{Y} - \mathbb{E}[y](\bar{W} - 1).
\label{eq:taylor_snips}
\end{align}

We can also write out an empirical estimate for $\beta$-IPS:
\begin{align}
 \hat{V}_{\beta{\rm -IPS}} &= \beta + \frac{1}{n}\sum w(r - \beta) \nonumber \\
 &= \beta + \bar{Y} - \beta\bar{W} \nonumber \\
 &= \bar{Y} - \beta(\bar{W}-1).
 \label{eq:bips}
\end{align}

Equations~\ref{eq:taylor_snips} and~\ref{eq:bips} show a fundamental equivalence between the SNIPS and $\beta$-IPS estimators.
Whereas $\beta$-IPS characterises the optimal variance-minimising value of $\beta$, SNIPS essentially uses an estimate for the expected policy value as a control variate.
Again, because we can prove that $\beta^{\star}$ is optimal, SNIPS can only ever happen to be lucky and recover the optimality of $\beta$-IPS, or provide a  fundamentally inferior estimator.

\textcolor{Maroon}{\it
The problem here is that we're not really talking about SNIPS, but about its first-order Taylor expansion.
The obvious question to ask is then, well, are we actually missing out on interesting higher-order behaviour that SNIPS has going for itself?
My gut says no, but I'm not an expert in these kinds of things at all. Do you think we can maybe bound how far we are off?
Could we actually show that for reasonable policies, it does not matter?
~\\
What does follow from this is that SNIPS' variance, in the way it is typically computed through the Delta method, will always be lower-bounded by $\beta$-IPS variance.
So: for all practical intents and purposes, $\beta$-IPS will yield lower variance.
The question is just whether the approximation we get from the Delta method can reasonably be justified.
Maybe there's a central limit theorem argument to be made for that, since the Delta method is equivalent to a normal approximation? (see Eq. 8 and surrounding text in \citet{Swaminathan2015})
~\\
I have empirically observed, repeatedly, that confidence intervals for SNIPS using the delta method variance estimate do actually exhibit nominal coverage levels, so that's a weak argument to say that it should be fine for large samples.
}
\textcolor{Blue}{1) Can we analytically compare the \it{approximate} variance of SNIPS with the variance of $\beta$-IPS? 2) The gaussian approximation is valid for large sample size, $N$, right? Then the comparison will also be only valid for large sample size.}
\textcolor{Maroon}{
I think that our $\beta^\star$ estimate corresponds to $\frac{{\rm Cov}(y,w)}{{\rm Var}(w)}$, and you can show that from Eq. 6, that's optimal. So either $\mathbb{E}[y]=\beta^\star$ due to luck, or SNIPS' variance is worse (asymptotically).
An asymptotic argument is already good, I think, no?
}
\textcolor{Blue}{I think so, yes. Then we just need to formalize this argument, right? i.e. , Var(SNIPS) $\geq$ Var($\beta$-IPS), asymptotically?}

\section{SNIPS vs $\beta$-IPS}
\textcolor{Maroon}{First attempt to prove that variance of SNIPS is higher than variance of beta-IPS.}

\textcolor{Maroon}{Check the following proof again.}

The variance of the $\beta$-IPS estimator can be given as:
\begin{equation}
\operatorname{Var}\!\bigl(\widehat{V}_{\beta\text{-IPS}}\bigr)
= \frac{1}{n}\Bigl(
      \sigma_{wr}^{2}
      - 2\beta\,\sigma_{w,wr}
      + \beta^{2}\sigma_w^{2}
  \Bigr)
\end{equation}
%
The optimal $\beta$ is given as~\cite{Gupta2024}:

\begin{equation}
\beta^{\star}
\;=\;
\frac{\sigma_{w,wr}}{\sigma_w^{2}}
\end{equation}

Plugging-in the optimal value, we get the following optimal (lowest) variance:
\begin{equation}\tag{2}
\operatorname{Var}\!\bigl(\widehat{V}_{\beta^{\star}\text{-IPS}}\bigr)
= \frac{1}{n}\left(
      \sigma_{wr}^{2}
      - \frac{\sigma_{w,wr}^{2}}{\sigma_w^{2}}
  \right)
\end{equation}


The variance of the SNIPS estimator (from the delta method) can be given as:
\begin{equation}\tag{3}
\operatorname{Var}\!\bigl(\widehat{V}_{\text{SNIPS}}\bigr)
\approx
\frac{1}{n}\Bigl(
      \sigma_{wr}^{2}
      + \mu^{2}\sigma_{w}^{2}
      - 2\mu\,\sigma_{w,wr}
  \Bigr)
\end{equation}

The difference in the variances is:
\begin{equation}\tag{4}
\Delta
=
\operatorname{Var}\!\bigl(\widehat{V}_{\text{SNIPS}}\bigr)
-
\operatorname{Var}\!\bigl(\widehat{V}_{\beta^{\star}\text{-IPS}}\bigr)
= \frac{1}{n}\,
  \frac{\bigl(\mu\,\sigma_{w}^{2} - \sigma_{w,wr}\bigr)^{2}}
       {\sigma_{w}^{2}}
\end{equation}

The variance of $\beta$-IPS is lower than SNIPS variance:

\begin{equation}
\operatorname{Var}\!\bigl(\widehat{V}_{\beta^{\star}\text{-IPS}}\bigr)
\;\le\;
\operatorname{Var}\!\bigl(\widehat{V}_{\text{SNIPS}}\bigr)
\end{equation}


Proof:
\begin{align}
\Delta
&=
\operatorname{Var}\!\bigl(\widehat{V}_{\text{SNIPS}}\bigr)
-
\operatorname{Var}\!\bigl(\widehat{V}_{\beta^{\star}\text{-IPS}}\bigr)\\
&=
\frac{1}{n}\left(
      \sigma_{wr}^{2}
      + \mu^{2}\sigma_{w}^{2}
      - 2\mu\,\sigma_{w,wr}
      - \sigma_{wr}^{2}
      + \frac{\sigma_{w,wr}^{2}}{\sigma_{w}^{2}}
\right)\\
&=
\frac{1}{n}\,
\frac{\bigl(\mu\,\sigma_{w}^{2} - \sigma_{w,wr}\bigr)^{2}}
     {\sigma_{w}^{2}}
\;\ge\;0.
\end{align}

\newpage

\begin{theorem}[Asymptotic MSE comparison of $\beta^{\*}$-IPS and SNIPS]
\label{thm:mse-betaips-snips}
Let $\{(x_i,a_i,r_i)\}_{i=1}^n$ be i.i.d.\ logged data generated under a logging
policy $\pi_0$. Let
$w_i=\pi(a_i\,|\,x_i)/\pi_0(a_i\,|\,x_i)$ be the importance weight for a target
policy $\pi$. Assume:
\begin{enumerate}
\item Rewards are bounded: $|r_i|\le R<\infty$.
\item Importance weights are bounded: $0\le w_i\le W<\infty$.
\item $\mathbb{E}[w_i]=1$ and $\mathbb{E}[w_i^2]<\infty$.
\end{enumerate}

Let $V(\pi)=\mathbb{E}[w_i r_i]$ denote the true policy value. Define
\[
\hat V_{\mathrm{SNIPS}}
=
\frac{\frac{1}{n}\sum_{i=1}^n w_i r_i}{\frac{1}{n}\sum_{i=1}^n w_i},
\qquad
\hat V_{\beta\mathrm{-IPS}}(\beta)
=
\beta + \frac{1}{n}\sum_{i=1}^n w_i(r_i-\beta).
\]
Let $\beta^{\*}$ denote the baseline that minimizes the mean squared error (MSE)
within the family of estimators with a global additive control variate
(cf.\ Eq.~(38) in~\cite{Gupta2024}). Then
\[
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(\beta^{\*})\right)
\le
\mathrm{MSE}\!\left(\hat V_{\mathrm{SNIPS}}\right) + O(n^{-2}),
\]
and in particular $\beta^{\*}$-IPS is asymptotically no worse in MSE than SNIPS.
Moreover, if $\beta^{\*}\neq V(\pi)$ and $\mathrm{Var}(w_i)>0$, the inequality is
strict for all sufficiently large $n$.
\end{theorem}

\begin{proof}
We write $V=V(\pi)$ for brevity and define the empirical means
\[
\bar X \triangleq \frac{1}{n}\sum_{i=1}^n w_i r_i,
\qquad
\bar W \triangleq \frac{1}{n}\sum_{i=1}^n w_i .
\]
Then $\hat V_{\mathrm{SNIPS}}=\bar X/\bar W$ and
\[
\hat V_{\beta\mathrm{-IPS}}(\beta)
=
\beta + \frac{1}{n}\sum_{i=1}^n w_i(r_i-\beta).
\]
In particular, for $\beta=V$,
\begin{equation}
\hat V_{\beta\mathrm{-IPS}}(V)
=
V + \bar X - V\bar W .
\label{eq:betaipsV}
\end{equation}

\medskip
\noindent\textbf{Step 1: Exact decomposition.}
Let $L_n \triangleq \bar X - V\bar W$. Using $\hat V_{\mathrm{SNIPS}}=\bar X/\bar W$
and~\eqref{eq:betaipsV}, we obtain the exact identity
\begin{align}
\hat V_{\mathrm{SNIPS}} - \hat V_{\beta\mathrm{-IPS}}(V)
&=
\frac{\bar X}{\bar W} - \bigl(V+\bar X - V\bar W\bigr) \nonumber\\
&=
L_n\Bigl(\frac{1}{\bar W}-1\Bigr) \nonumber\\
&=
L_n\cdot \frac{1-\bar W}{\bar W}. \label{eq:Rn}
\end{align}
Define the remainder random variable
\[
R_n \triangleq L_n\cdot \frac{1-\bar W}{\bar W}.
\]
Then
\[
\hat V_{\mathrm{SNIPS}}
=
\hat V_{\beta\mathrm{-IPS}}(V) + R_n .
\]

\medskip
\noindent\textbf{Step 2: Bounding the remainder.}
Let $\mathcal{E}=\{\bar W\ge 1/2\}$. Since $0\le w_i\le W$ and
$\mathbb{E}[w_i]=1$, Hoeffding’s inequality gives
\[
\mathbb{P}(\mathcal{E}^c)
=
\mathbb{P}(\bar W-1\le -1/2)
\le
\exp\!\Bigl(-\frac{n}{2W^2}\Bigr).
\]
On $\mathcal{E}$ we have $\bar W\ge 1/2$ and hence
\[
\Bigl|\frac{1-\bar W}{\bar W}\Bigr|\le 2|1-\bar W|.
\]
Therefore, on $\mathcal{E}$,
\[
R_n^2 \le 4 L_n^2(1-\bar W)^2 .
\]
Splitting expectations on $\mathcal{E}$ yields
\begin{align}
\mathbb{E}[R_n^2]
&\le
4\,\mathbb{E}\!\left[L_n^2(1-\bar W)^2\right]
+
\mathbb{E}\!\left[R_n^2\mathbf{1}\{\mathcal{E}^c\}\right].
\label{eq:split}
\end{align}

Define $U_i=w_i r_i - Vw_i$ and $T_i=w_i-1$. Then
$L_n=\frac{1}{n}\sum_{i=1}^n U_i$ and $1-\bar W=-\frac{1}{n}\sum_{i=1}^n T_i$.
Using $|r_i|\le R$, $0\le w_i\le W$, and $|V|\le WR$, we have
$|U_i|\le RW(1+W)$ and $|T_i|\le W$. Since $(U_i)$ and $(T_i)$ are bounded,
mean-zero, and i.i.d., standard fourth-moment bounds for averages imply the
existence of constants $C_U,C_T<\infty$ such that
\[
\mathbb{E}[L_n^4] \le \frac{C_U}{n^2},
\qquad
\mathbb{E}[(1-\bar W)^4] \le \frac{C_T}{n^2}.
\]
By Cauchy--Schwarz,
\[
\mathbb{E}\!\left[L_n^2(1-\bar W)^2\right]
\le
\sqrt{\mathbb{E}[L_n^4]}\sqrt{\mathbb{E}[(1-\bar W)^4]}
\le
\frac{\sqrt{C_U C_T}}{n^2}.
\]

Under boundedness and the standard positivity assumption
$\pi_0(a|x)>0$ whenever $\pi(a|x)>0$, $R_n^2$ is almost surely finite.
Hence there exists $K<\infty$ such that
\[
\mathbb{E}\!\left[R_n^2\mathbf{1}\{\mathcal{E}^c\}\right]
\le
K\,\mathbb{P}(\mathcal{E}^c)
\le
K\exp\!\Bigl(-\frac{n}{2W^2}\Bigr).
\]
Combining with~\eqref{eq:split} yields
\[
\mathbb{E}[R_n^2]=O(n^{-2}).
\]

\medskip
\noindent\textbf{Step 3: MSE expansion.}
From $\hat V_{\mathrm{SNIPS}}=\hat V_{\beta\mathrm{-IPS}}(V)+R_n$ we have
\[
\hat V_{\mathrm{SNIPS}}-V
=
\bigl(\hat V_{\beta\mathrm{-IPS}}(V)-V\bigr)+R_n .
\]
Therefore,
\begin{align*}
\mathrm{MSE}(\hat V_{\mathrm{SNIPS}})
&=
\mathbb{E}\!\left[\bigl(\hat V_{\mathrm{SNIPS}}-V\bigr)^2\right] \\
&=
\mathbb{E}\!\left[\bigl(\hat V_{\beta\mathrm{-IPS}}(V)-V\bigr)^2\right]
+2\mathbb{E}\!\left[\bigl(\hat V_{\beta\mathrm{-IPS}}(V)-V\bigr)R_n\right]
+\mathbb{E}[R_n^2].
\end{align*}
By Cauchy--Schwarz,
\[
\Bigl|\mathbb{E}\!\left[\bigl(\hat V_{\beta\mathrm{-IPS}}(V)-V\bigr)R_n\right]\Bigr|
\le
\sqrt{\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(V)\right)}
\sqrt{\mathbb{E}[R_n^2]} .
\]
Since $\mathrm{MSE}(\hat V_{\beta\mathrm{-IPS}}(V))=O(1/n)$ and
{\color{blue}
$\mathbb{E}[R_n^2]=O(1/n^2)$, the cross term is $O(n^{-3/2})$ and negligible.
\textcolor{Maroon}{{Not sure about this claim :- $O(n^{-3/2})$ and negligible.}}
}
Hence
\[
\mathrm{MSE}(\hat V_{\mathrm{SNIPS}})
=
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(V)\right)
+ O(n^{-2}).
\]

\medskip
\noindent\textbf{Step 4: Comparison with the optimal baseline.}
By Theorem~2 of~\cite{Gupta2024}, $\beta^*$-IPS minimizes the MSE within the
class of offline estimators with a global additive control variate. Therefore,
\[
\mathrm{MSE}\left(\hat{V}_{\beta-\mathrm{IPS}}(\beta^*)\right)
\le
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(V)\right).
\]
Combining with the previous step gives
\[
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(\beta^*)\right)
\le
\mathrm{MSE}\!\left(\hat V_{\mathrm{SNIPS}}\right) + O(n^{-2}).
\]

Finally, if $\beta^{\*}\neq V$ and $\mathrm{Var}(w_i)>0$, the gap between the two
additive estimators is of order $1/n$ whereas the remainder term is of order
$1/n^2$, implying strict dominance of $\beta^{\*}$-IPS over SNIPS for all
sufficiently large $n$.
\end{proof}

\newpage

\section{Version without probabilistic bounds used in Step 2, assuming clipped weights}

\begin{theorem}[Asymptotic MSE comparison under clipped weights]
\label{thm:mse-clipped-on2}
Let $\{(x_i,a_i,r_i)\}_{i=1}^n$ be i.i.d.\ logged data generated under a logging
policy $\pi_0$. Let
$w_i=\pi(a_i\,|\,x_i)/\pi_0(a_i\,|\,x_i)$ be the importance weight for a target
policy $\pi$. Assume:
\begin{enumerate}
\item Rewards are bounded: $|r_i|\le R<\infty$.
\item Weights are clipped: $w_i\in[w_{\min},W]$ for some $0<w_{\min}\le W<\infty$.
\item $\mathbb{E}[w_i]=1$.
\end{enumerate}
Let $V(\pi)=\mathbb{E}[w_i r_i]$ denote the true policy value. Define
\[
\hat V_{\mathrm{SNIPS}}
=
\frac{\frac{1}{n}\sum_{i=1}^n w_i r_i}{\frac{1}{n}\sum_{i=1}^n w_i},
\qquad
\hat V_{\beta\mathrm{-IPS}}(\beta)
=
\beta + \frac{1}{n}\sum_{i=1}^n w_i(r_i-\beta).
\]
Let $\beta^{\*}$ denote the baseline minimizing the MSE among all estimators with a
global additive control variate (as in \cite{gupta2024optimal}). Then
\[
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(\beta^{\*})\right)
\le
\mathrm{MSE}\!\left(\hat V_{\mathrm{SNIPS}}\right) + O(n^{-2}),
\]
and hence $\beta^{\*}$-IPS is asymptotically no worse in MSE than SNIPS.
\end{theorem}

\begin{proof}
We write $V=V(\pi)$ and define empirical means
\[
\bar X = \frac{1}{n}\sum_{i=1}^n w_i r_i,
\qquad
\bar W = \frac{1}{n}\sum_{i=1}^n w_i .
\]
Then $\hat V_{\mathrm{SNIPS}}=\bar X/\bar W$ and
\[
\hat V_{\beta\mathrm{-IPS}}(\beta)
=
\beta + \frac{1}{n}\sum_{i=1}^n w_i(r_i-\beta).
\]
In particular, for $\beta=V$,
\begin{equation}
\hat V_{\beta\mathrm{-IPS}}(V)
=
V + \bar X - V\bar W .
\label{eq:betaV-on2}
\end{equation}

\medskip
\noindent\textbf{Step 1: Exact decomposition.}
Using $\hat V_{\mathrm{SNIPS}}=\bar X/\bar W$ and~\eqref{eq:betaV-on2}, we obtain
\begin{align}
\hat V_{\mathrm{SNIPS}} - \hat V_{\beta\mathrm{-IPS}}(V)
&=
\frac{\bar X}{\bar W} - (V + \bar X - V\bar W) \nonumber\\
&=
(\bar X - V\bar W)\Bigl(\frac{1}{\bar W}-1\Bigr) \nonumber\\
&=
(\bar X - V\bar W)\cdot\frac{1-\bar W}{\bar W}.
\label{eq:decomp-on2}
\end{align}
Define
\[
R_n \triangleq (\bar X - V\bar W)\cdot\frac{1-\bar W}{\bar W}.
\]
Then
\[
\hat V_{\mathrm{SNIPS}}
=
\hat V_{\beta\mathrm{-IPS}}(V) + R_n .
\]

\medskip
\noindent\textbf{Step 2: Bounding $\mathbb{E}[R_n^2]$ (dependence-safe).}
Define
\[
L_n \triangleq \bar X - V\bar W,
\qquad
\Delta_n \triangleq 1-\bar W,
\]
so that $R_n = L_n\Delta_n/\bar W$.
By clipped weights, $\bar W\in[w_{\min},W]$ almost surely, hence
$1/\bar W^2 \le 1/w_{\min}^2$. Therefore,
\begin{equation}
R_n^2
=
\frac{L_n^2\Delta_n^2}{\bar W^2}
\le
\frac{1}{w_{\min}^2}\,L_n^2\Delta_n^2.
\label{eq:Rn-bound-on2}
\end{equation}
Taking expectations and applying Cauchy--Schwarz,
\begin{equation}
\mathbb{E}[R_n^2]
\le
\frac{1}{w_{\min}^2}\,
\sqrt{\mathbb{E}[L_n^4]}\,
\sqrt{\mathbb{E}[\Delta_n^4]}.
\label{eq:CS-on2}
\end{equation}

Let
\[
U_i \triangleq w_i r_i - V w_i,
\qquad
T_i \triangleq 1-w_i.
\]
Then $L_n=\frac{1}{n}\sum_{i=1}^n U_i$ and $\Delta_n=\frac{1}{n}\sum_{i=1}^n T_i$.
Moreover, $\mathbb{E}[U_i]=0$ and $\mathbb{E}[T_i]=\mathbb{E}[1-w_i]=0$.
Since $|r_i|\le R$ and $w_i\in[w_{\min},W]$, both $U_i$ and $T_i$ are bounded
and therefore have finite fourth moments.

For i.i.d.\ mean-zero random variables $Z_i$ with $\mathbb{E}[Z_1^4]<\infty$,
\begin{equation}
\mathbb{E}\!\left[\left(\frac{1}{n}\sum_{i=1}^n Z_i\right)^4\right]
=
\frac{1}{n^4}\Bigl(n\mathbb{E}[Z_1^4]
+ 3n(n-1)(\mathbb{E}[Z_1^2])^2\Bigr)
= O(n^{-2}).
\label{eq:fourth-moment-on2}
\end{equation}
Applying~\eqref{eq:fourth-moment-on2} to $Z_i=U_i$ and $Z_i=T_i$ gives
\[
\mathbb{E}[L_n^4]=O(n^{-2}),
\qquad
\mathbb{E}[\Delta_n^4]=O(n^{-2}).
\]
Substituting into~\eqref{eq:CS-on2} yields
\begin{equation}
\mathbb{E}[R_n^2] = O(n^{-2}).
\label{eq:Rn2-on2}
\end{equation}

\medskip
\noindent\textbf{Step 3: MSE expansion with an $O(n^{-2})$ cross-term.}
Write
\[
\hat V_{\mathrm{SNIPS}}-V = A_n + R_n,
\qquad
A_n \triangleq \hat V_{\beta\mathrm{-IPS}}(V)-V = L_n.
\]
Then
\begin{equation}
\mathrm{MSE}(\hat V_{\mathrm{SNIPS}})
=
\mathbb{E}[A_n^2] + 2\mathbb{E}[A_nR_n] + \mathbb{E}[R_n^2].
\label{eq:mse-expand-on2}
\end{equation}
We bound the cross term $\mathbb{E}[A_nR_n]=\mathbb{E}[L_nR_n]$ more sharply than
Cauchy--Schwarz by exploiting cancellations.

Since $R_n=L_n\Delta_n/\bar W$ and $\bar W = 1-\Delta_n$, we have
\[
\mathbb{E}[A_nR_n]
=
\mathbb{E}\!\left[\frac{L_n^2\Delta_n}{\bar W}\right]
=
\mathbb{E}\!\left[\frac{L_n^2\Delta_n}{1-\Delta_n}\right].
\]
Using the exact identity
\[
\frac{1}{1-\Delta_n} = 1 + \Delta_n + \frac{\Delta_n^2}{1-\Delta_n}
\qquad
(\text{valid since }\bar W\ge w_{\min}>0),
\]
we obtain
\begin{equation}
\mathbb{E}[A_nR_n]
=
\mathbb{E}[L_n^2\Delta_n]
+
\mathbb{E}[L_n^2\Delta_n^2]
+
\mathbb{E}\!\left[\frac{L_n^2\Delta_n^3}{\bar W}\right].
\label{eq:cross-decomp-on2}
\end{equation}

\emph{Bounding $\mathbb{E}[L_n^2\Delta_n^2]$.}
By Cauchy--Schwarz and the fourth-moment bounds above,
\[
\mathbb{E}[L_n^2\Delta_n^2]
\le
\sqrt{\mathbb{E}[L_n^4]}\sqrt{\mathbb{E}[\Delta_n^4]}
=
O(n^{-2}).
\]

\emph{Bounding $\mathbb{E}[\frac{L_n^2\Delta_n^3}{\bar W}]$.}
Since $\bar W\ge w_{\min}$,
\[
\mathbb{E}\!\left[\left|\frac{L_n^2\Delta_n^3}{\bar W}\right|\right]
\le
\frac{1}{w_{\min}}\,\mathbb{E}\!\left[|L_n|^2|\Delta_n|^3\right]
\le
\frac{1}{w_{\min}}\sqrt{\mathbb{E}[L_n^4]}\sqrt{\mathbb{E}[\Delta_n^6]}.
\]
Because $T_i$ is bounded, the same sample-mean moment calculation implies
$\mathbb{E}[\Delta_n^6]=O(n^{-3})$. Together with $\mathbb{E}[L_n^4]=O(n^{-2})$,
this gives
\[
\mathbb{E}\!\left[\frac{L_n^2\Delta_n^3}{\bar W}\right] = O(n^{-5/2}).
\]

\emph{Bounding $\mathbb{E}[L_n^2\Delta_n]$ by index cancellation.}
Recall $L_n=\frac{1}{n}\sum_i U_i$ and $\Delta_n=\frac{1}{n}\sum_k T_k$ where
$U_i=w_ir_i-Vw_i$ and $T_i=1-w_i$. Then
\[
\mathbb{E}[L_n^2\Delta_n]
=
\frac{1}{n^3}\sum_{i,j,k}\mathbb{E}[U_iU_jT_k].
\]
By independence across indices and $\mathbb{E}[U_i]=\mathbb{E}[T_i]=0$,
$\mathbb{E}[U_iU_jT_k]=0$ unless $i=j=k$. Therefore,
\[
\mathbb{E}[L_n^2\Delta_n]
=
\frac{1}{n^3}\sum_{i=1}^n \mathbb{E}[U_i^2T_i]
=
\frac{n\,\mathbb{E}[U_1^2T_1]}{n^3}
=
O(n^{-2}).
\]
Combining the three bounds in~\eqref{eq:cross-decomp-on2} yields
\begin{equation}
\mathbb{E}[A_nR_n] = O(n^{-2}).
\label{eq:cross-on2}
\end{equation}

Substituting~\eqref{eq:Rn2-on2} and~\eqref{eq:cross-on2} into~\eqref{eq:mse-expand-on2}
gives
\[
\mathrm{MSE}(\hat V_{\mathrm{SNIPS}})
=
\mathbb{E}[A_n^2] + O(n^{-2})
=
\mathrm{MSE}(\hat V_{\beta\mathrm{-IPS}}(V)) + O(n^{-2}).
\]

\medskip
\noindent\textbf{Step 4: Comparison with the optimal baseline.}
By Theorem~2 in \cite{gupta2024optimal}, $\beta^{\*}$-IPS minimizes the MSE
within the class of global additive control variate estimators. Hence,
\[
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(\beta^{\*})\right)
\le
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(V)\right).
\]
Combining with the previous display yields
\[
\mathrm{MSE}\!\left(\hat V_{\beta\mathrm{-IPS}}(\beta^{\*})\right)
\le
\mathrm{MSE}\!\left(\hat V_{\mathrm{SNIPS}}\right) + O(n^{-2}),
\]
which completes the proof.
\end{proof}














